Parallelizing Thompson Sampling

How can we make use of information parallelism in online decision making problems while efficiently balancing the exploration-exploitation trade-off? In this paper, we introduce a batch Thompson Sampling framework for two canonical online decision making problems, namely, stochastic multi-arm bandit and linear contextual bandit with finitely many arms. Over a time horizon $T$, our \textit{batch} Thompson Sampling policy achieves the same (asymptotic) regret bound of a fully sequential one while carrying out only $O(\log T)$ batch queries. To achieve this exponential reduction, i.e., reducing the number of interactions from $T$ to $O(\log T)$, our batch policy dynamically determines the duration of each batch in order to balance the exploration-exploitation trade-off. We also demonstrate experimentally that dynamic batch allocation dramatically outperforms natural baselines such as static batch allocations.

==> analysis.tex <==
\begin{theorem}
Let $\delta \in (0,1)$ be the target error probability. To achieve expected error probability less than $\delta$, it suffices to run $ECED$, the following number of iterations 
\[
O(\frac{k}{c_{\epsilon}}(\log \frac{kn(1+\epsilon)}{\delta} \log\frac{n(1+\epsilon)}{\delta})^2 ).
\]

\end{theorem}
\begin{proof}
Let $\psi_{\ell}$ be a path ending up at level $\ell$ of the semi-adaptive algorithm. 
%Let $e=\arg\max_{e'} \Delta_{ECED}(X_{e'}|\psi_{\ell})$.

After running $OPT(\delta_{opt})$,
from Lemma~\ref{lem:lem2}, we have $f_{AUX}^{avg}(OPT(\delta_{opt})).4\log(n/\delta_g) \ge \delta_{opt}.c_{\delta}$.
Then,
\begin{align*} 
    &(f_{AUX}^{avg}(\ell)-f_{AUX}^{avg}(OPT(\delta_{opt})).4\log \frac{n}{\delta_g}).\frac{c_{\epsilon}}{kc_{\delta}}-c_{\eta,\epsilon}
     \\
    \le & \Ex_{\psi_{\ell}}[\Delta_{AUX}(e|\psi) | e=\arg\max_{e'} \Delta_{ECED}(e'|\psi_{\ell})] \\
    = &   \Ex_{\bar{\psi}} [\Ex_{\psi_{\ell} \succeq \bar{\psi}} [\Delta_{AUX}(e|\psi_{\ell}) | e=\arg\max_{e'} \Delta_{ECED}(e'|\psi_{\ell})]]\\
    \le & \Ex_{\bar{\psi}}[\frac{1}{1+\epsilon} \Ex_{\psi_{\ell} \succeq \bar{\psi}} [ \Delta_{AUX} (e|\psi_{\ell})] | e=\max_{e'} \Ex_{\psi^{\pi}_{\ell} \succeq \bar{\psi}}[\Delta_{ECED}(e'|\psi^{\pi}_{\ell})]]\\
    =&\frac{1}{1+\epsilon} \Ex_{\bar{\psi}}[ \Ex_{\psi_{\ell}\succeq \bar{\psi}} [ \Delta_{AUX} (e|\psi_{\ell})] | e=\max_{e'} \Ex_{\psi^{\pi}_{\ell} \succeq \bar{\psi}}[\Delta_{ECED}(e'|\psi^{\pi}_{\ell})]]\\
    %= & \frac{1}{1+\epsilon} \Ex_{\psi_{\ell}}[\Delta_{AUX}(e|\psi_{\ell}) | e= \arg\max_{e'} \Delta_{ECED}(e'|\psi_{\ell})]\\
    = & \frac{1}{1+\epsilon}
    (f_{AUX}^{avg}(\ell) - f_{AUX}^{avg}(\ell+1)).
\end{align*}
The first inequality is from~\cite{Chen_2017}. The third inequality is by information gap definition. The last equality is based on the algorithm description and semi-adaptive value.

Now let $\Delta_{\ell} = f_{AUX}^{avg}(\ell) - f_{AUX}^{avg} (OPT(\delta_{opt})).4\log \frac{n}{\delta_g}$. Therefore, 
\[
\frac{1}{1+ \epsilon}(\Delta_{\ell}-\Delta_{\ell+1}) \ge \Delta_{\ell}.\frac{c_{\epsilon}}{kc_{\delta}}-c_{\eta,\epsilon}.
\]
Thus $\Delta_{\ell+1} \le \Delta_{\ell} (1-\frac{(1+\epsilon) c_{\epsilon}}{kc_{\delta}}) + (1+\epsilon) c_{\eta,\epsilon}$. Hence
\[
\Delta_{k'} \le exp(-k'\frac{c_{\epsilon}}{kc_{\delta}}(1+\epsilon)) \Delta_0 + \frac{kc_{\delta}}{c_{\epsilon}}.c_{\eta,\epsilon}(1+\epsilon).
\]
Now by following the steps in the proof of Theorem 1 in~\cite{Chen_2017}, 
by setting $k'$ and $\delta_{opt}$ as in eq. (B.28),
we can get $f_{AUX}^{avg} (k') \le 2c.\delta_g (1+\epsilon)$. Thus by Lemma~\ref{lem:lem2} we get $p_{ERR} \le \delta_g(1+\epsilon)$.
Similar to~\cite{Chen_2017}, the exact value of $k'$ can be computed as $O(\frac{k}{c_{\epsilon}}(\log \frac{kn(1+\epsilon)}{\delta} \log\frac{n(1+\epsilon)}{\delta})^2 )$.

\end{proof}



l

\subsection{Query Complexity}


==> checklist.tex <==
\section*{Checklist}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section 4.3}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{No negative societal impact.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
  \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{In supplemental.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{For more details, see the supplemental}
  \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We plot the result with 1 std error in shade.}
  \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Please check the supplemental.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

